Inference after latent variable estimation for single-cell RNA sequencing data

In the analysis of single-cell RNA sequencing data, researchers often characterize the variation between cells by estimating a latent variable, such as cell type or pseudotime, representing some aspect of the individual cell's state. They then test each gene for association with the estimated latent variable. If the same data are used for both of these steps, then standard methods for computing p-values and confidence intervals in the second step will fail to achieve statistical guarantees such as Type 1 error control. Furthermore, approaches such as sample splitting that can be applied to solve similar problems in other settings are not applicable in this context. In this paper, we introduce count splitting, a flexible framework that allows us to carry out valid inference in this setting, for virtually any latent variable estimation technique and inference approach, under a Poisson assumption. We demonstrate the Type 1 error control and power of count splitting in a simulation study, and apply count splitting to a dataset of pluripotent stem cells differentiating to cardiomyocytes.

==> Sections/section3-old.tex <==
\section{Existing methods for latent variable inference}
\label{section_existingmethods}

\subsection{Motivating Example}
\label{subsec_motivatingexample}

%%% Should I mention that this is a global null where not even size factors cause differences between cells or genes?
Throughout Section~\ref{section_existingmethods}, we refer to a toy example to compare existing methods for differential expression analysis after latent variable estimation. We generate $2,000$ realizations of $\bold{X} \in \mathbb{R}^{200 \times 10}$, where $\bold{X}_{i,j} \overset{ind.}{\sim} \text{Poisson}(\Lambda_{ij})$. For $i = 1,\ldots,200$, we let $\Lambda_{ij}=1$ for $j = 1,\ldots,5$ and $\Lambda_{ij}=10$ for $j = 6,\ldots,10$. 
For each realized dataset $X$, we estimate the developmental trajectory by letting 
$\hat{L}(X)$ be the first principal component of the log-transformed data \citep{ashenberg2019models}. 
We then fit Poisson GLMs are rely on Wald p-values for differential expression analysis. Since all columns of $\Lambda$ are constant, $\beta_{1}(Z, \bold{X}_j)=0$ for all $j$ and for any $Z$. 
Therefore, all p-values computed for differential expression should follow a $\text{Unif}(0,1)$ distribution. As we show throughout this section, for most existing methods
for carrying out differential expression analysis the p-values either cannot be computed or fail to meet this criterion. 

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{Figures/Fig1.png}
\caption{Uniform QQ-plots of p-values for the $p=10$ genes in each of 2000 datasets generated as described in Section~\ref{subsec_motivatingexample}. The left-hand panel shows all of the genes aggregated, whereas the center and right panels break the results down by the value of $\Lambda_{ij}$.}
\label{fig_globalnull}
\end{figure}

\subsection{Naive method}
\label{subsec_naive}

The ``naive method" refers to using the same data for latent variable estimation and differential expression analysis, 
without correcting for this double use.
Using notation from Section~\ref{section_background}, this means attempting to do inference on the parameters $ \beta_1\left( \hat{L}(X), \bold{X}_j\right)$ in \eqref{eq_betadef} by regressing $X_j$ on $\hat{L}(X)$. The Wald p-values computed for this GLM have the form
\begin{equation}
\label{eq_naivep}
\text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X),\bold{X}_j\right)=0} \left( 
\left| 
\widehat{\beta}_{1}\left(\hat{L}(X),\bold{X}_j\right) \right|
  \geq 
  \left| 
  \widehat{\beta}_{1}\left(\hat{L}\left(X\right), X_j\right) \right|
 \right).
\end{equation}
The problem with \eqref{eq_naivep} is that the left-hand side of the inequality is a double-dipped coefficient (as defined in Section~\ref{section_background}) while the right-hand side is not. Since the observed realization $X_j$ contributed to the construction of $\hat{L}(X)$, even when the null hypothesis holds, the estimated coefficient $\widehat{\beta}_{1}\left(\hat{L}(X),\bold{X}_j\right)$ looks artificially large compared to the distribution of $\widehat{\beta}_{1}\left(\hat{L}(X),\bold{X}_j\right)$. Thus, under the null hypothesis, if we compute the p-value in \eqref{eq_naivep} for many realizations of $X$ under the null, the collection of p-values will be stochastically dominated by the $\text{Unif}(0,1)$ distribution and will thus fail to control the Type 1 error (Figure~\ref{fig_globalnull}). 


\subsection{Cell Splitting}
\label{subsec_sampsplit}

In some settings, splitting the observations in a sample into a training set and a testing set can provide a simple way to avoid using the same dataset to generate and then test a hypothesis. However, in the setting of this paper, splitting the cells in $X$ does not allow us to bypass the issues of double dipping.

The issue arises in obtaining latent variable coordinates for the cells in $X^{test}$ using the cells in $X^{train}$. In our simple principal component example, one could compute the first principal axis of the log-transformed $X^{train}$ matrix, and then project the log-transformed $X^{test}$ onto this axis to obtain coordinates for the cells in $X^{test}$. Unfortunately, this projection step involves using the data in $X^{test}$. The p-value from cell-splitting thus has the form
\footnotesize
\begin{equation}
\label{eq_cellsplitp}
\text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X^{train}, X^{test}),\bold{X}^{test}_j\right)=0} \left( 
\left| 
\widehat{\beta}_{1}\left(\hat{L}({X}^{train}, X^{test}),\bold{X}^{test}_j\right) \right|
  \geq 
  \left| 
  \widehat{\beta}_{1}\left(\hat{L}\left(X^{train}, X^{test}\right), X_j^{test}\right) \right| \right),
\end{equation}
\normalsize
and suffers from the same issue as \eqref{eq_naivep}: the right-hand side of the inequality is a double-dipped coefficient while the left-hand side is not. Thus, over repeated realizations of $X$ under the null, the p-values from \eqref{eq_cellsplitp} do not follow a $\text{Unif}(0,1)$ distribution, and instead are anti-conservative, as shown in Figure~\ref{fig_globalnull}.

We briefly note that one might also consider forming two matrices $X^{train}$ and $X^{test}$ by splitting the genes (features) rather than the observations. In this setting, $\hat{L}\left(X^{train}\right)$ provides coordinates for all cells in $X$, and we can obtain p-values for each gene $X_j$ that is not in $X^{train}$ by regressing $X_j$ on $\hat{L}(X^{train})$. Then the roles of $X^{train}$ and $X^{test}$ can be swapped to obtain p-values for the remaining genes. Gene splitting therefore computes p-values of the form
\small
\begin{equation*}
\begin{cases}
	\text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X^{train}),\bold{X}^{test}_j\right)=0} \left( 
\left| 
\widehat{\beta}_{1}\left(\hat{L}(X^{train}),\bold{X}^{test}_j\right) \right|
  \geq 
  \left| 
  \widehat{\beta}_{1}\left(\hat{L}\left(X^{train}\right), X_j^{test}\right) \right| \right)  & \text{ if } X_j \in X^{test}, \\
  \text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X^{test}),\bold{X}^{train}_j\right)=0} \left( 
\left| 
\widehat{\beta}_{1}\left(\hat{L}({X}^{test}),\bold{X}^{train}_j\right) \right|
  \geq 
  \left| 
  \widehat{\beta}_{1}\left(\hat{L}\left(X^{test}\right), X_j^{train}\right) \right| \right) & \text{ if } X_j \in X^{train}.
\end{cases}.
\end{equation*}
While these p-values will be uniformly distributed over repeated realizations of $X$, they are fundamentally unsatisfactory in scRNA-seq applications where we wish to obtain a p-value for every gene \emph{with respect to the same estimated latent variable.} 

\subsection{Selective inference through conditioning}
\label{subsec_selective}

We next consider taking a selective inference approach \citep{taylor2015statistical} to correct the p-values in \eqref{eq_naivep}. This involves fitting the same regression model as the naive method, but replacing~\eqref{eq_naivep} with the conditional probability 
\begin{align}
\label{eq_selectivep}
\text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X),\bold{X}_j\right)=0} \left( \left| \widehat{\beta}_{1}\left(\hat{L}(X),\bold{X}_j\right) \right| \geq \left| \widehat{\beta}_{1}\left(\hat{L}\left(X\right), X_j\right) \right| \mid \hat{L}\left(\bold{X}\right) = \hat{L}(X) \right).
\end{align}
The inequality in \eqref{eq_selectivep} is identical to that in \eqref{eq_naivep}, but under the conditioning event,  \eqref{eq_selectivep} can be rewritten as 
\begin{align}
\label{eq_selectivep2}
\text{Pr}_{H_0:\  \beta_1\left(\hat{L}(X),\bold{X}_j\right)=0} \left( \left| \widehat{\beta}_{1}\left(\hat{L}(\bold{X}),\bold{X}_j\right) \right| \geq \left| \widehat{\beta}_{1}\left(\hat{L}\left(X\right), X_j\right) \right| \mid \hat{L}\left(\bold{X}\right) = \hat{L}(X) \right).
\end{align}
As both the left-hand and right-hand sides of the inequality are double-dipped coefficients in \eqref{eq_selectivep2}, over repeated realizations of $X$ under the null, the p-values in \eqref{eq_selectivep} follow a $\text{Unif}(0,1)$ distribution and thus control the Type 1 error. 

However, it is not clear how to compute \eqref{eq_selectivep}. 
The selective inference literature typically assumes normally distributed data. This assumption, along with extra conditioning, allows p-values similar to the one in \eqref{eq_selectivep} to be computed from a truncated Gaussian distribution. 
However, as scRNA-seq data consists of non-negative integers whose variance scales with the mean, a normality assumption is not suitable.
Furthermore, as explained in \cite{tian2018selective}, the fact that coefficient estimates in a GLM are asymptotically normal does not guarantee that they will be asymptotically truncated-normal after accounting for a conditioning event. 
Due to this difficulty, existing work on selective inference for GLMs has been more specialized, and either relies on specific forms for the conditioning event (not applicable to existing latent variable estimation techniques) or is restricted to a low-dimensional regime ($n \gg p$) \citep{taylor2018post, tibshirani2018uniform}. 

The fact that selective inference approaches require  explicit characterization of the conditioning event $\hat{L}(\bold{X}) = \hat{L}(X)$ for any $\hat{L}(\cdot)$ that we might want to use is particularly 
problematic in the scRNA-seq setting, where a huge number of specialized and complicated techniques are used for data pre-processing, clustering, and trajectory estimation. 

\cite{zhang2019valid} combine cell splitting with selective inference to obtain approximately valid p-values for differential expression of genes across clusters of cells in the scRNA-seq setting. They condition on the test-set labeling event $\hat{L}\left(X^{train}, \bold{X}^{test}\right) = \hat{L}\left(X^{train}, X^{test}\right)$, which in their particular framework is easier to characterize than the full selective inference event $\hat{L}\left(\bold{X}\right) = \hat{L}(X)$. Unfortunately, this method  assumes normally-distributed data and linearly separable clusters, and it does not extend naturally to the setting of trajectory estimation. \todo{This Zhang paragraph really seems to disrupt the flow. We need to cite them, but I would love to flow straight from "hard to compute conditioning event" into the "almost Jackstraw" stuff.}

Selective inference is omitted as a comparison method in Figure~\ref{fig_globalnull} because we are not aware of a way to compute \eqref{eq_selectivep} for Poisson data, even for a very simple choice of function $\hat{L}\left(\cdot\right)$.

As much of the difficulty with selective inference approaches lies in computing the conditioning event, another strategy is to try to directly approximate the marginal distribution of the double-dipped coefficient $\widehat{\beta}_{1}\left(\hat{L}(\bold{X}),\bold{X}_j\right)$, and thus compute a p-value of the form 
\begin{align}
\label{eq_almost_jackstraw}
\text{Pr}_{H_0: \beta_1\left(\hat{L}(X),\bold{X}_j\right)=0} \left( \left| \widehat{\beta}_{1}\left(\hat{L}(\bold{X}),\bold{X}_j\right) \right| \geq \left| \widehat{\beta}_{1}\left(\hat{L}\left(X\right), X_j\right) \right| \right).
\end{align}
Distributions of double-dipped coefficients such as $\widehat{\beta}_{1}\left(\hat{L}(\bold{X}),\bold{X}_j\right)$ typically are not analytically tractable, and it is not clear how to simulate a null distribution for $H_0: \beta_1\left(\hat{L}(X),\bold{X}_j\right)=0$ to compute an empirical approximation to \eqref{eq_almost_jackstraw}. In the next section, we discuss a framework that uses permutations to approximate the distribution of $\widehat{\beta}_{1}\left(\hat{L}(\bold{X}),\bold{X}_j\right)$, but does so under a slightly different null hypothesis. 

\subsection{Jackstraw}

The \emph{jackstraw} method of \cite{chung2015statistical} uses permutations to test for association between the principal components and features of a data matrix. The jackstraw framework was later extended to apply to additional latent variable estimation techniques, including clustering \citep{chung2020statistical}. To make our discussion of jackstraw congruent with the rest of this paper, we instantiate the framework to our latent variable GLM setting. We elaborate on the exact implementation of Jackstraw used in this paper in Appendix~\ref{appendix_fig1help}.
 

To test if the $j$th gene is differentially expressed, jackstraw creates datasets $X^{permute, b}$ for $b=1,\ldots,B$. Each dataset $X^{permute, b}$ is identical to $X$, but with the $j$th column randomly permuted. Each dataset gives rise to a GLM coefficient $\hat{\beta}\left(\hat{L}(X^{permute,b}),{X}^{permute,b}_j \right)$. The p-value is computed as
\begin{equation}
\label{jackstraw_empirical}
\frac{1}{B} \sum_{b=1}^B \bold{1} \left\{ \left| \hat{\beta}\left(\hat{L}(X^{permute,b}),{X}^{permute,b}_j \right) \right|	  \geq \left| \hat{\beta}\left(\hat{L}(X),{X}_j \right) \right|  \right\}.
\end{equation}

Under the null that $\beta_{1j} = \bold{0}$ in \eqref{eq_meanmodel}, $\bold{X}_{1j},\ldots,\bold{X}_{nj}$ are i.i.d. and the likelihood of $\bold{X}$ is invariant to permutation of the ordering of the entries in the $j$th column. 
Under this null, the distribution of $\hat{\beta}\left(\hat{L}(X^{permute,b}),{X}^{permute,b}_j \right)$ approximates that of the double dipped coefficient $\hat{\beta}\left(\hat{L}(\bold{X}),\bold{X}_j \right)$. Thus, over repeated realizations of $X$ under the null that $\beta_{1j} = \bold{0}$, the Jackstraw p-values for the $j$th gene follow a $\text{Unif}(0,1)$ distribution. We note that this null is slightly different than the ones tested in Sections~\ref{subsec_naive}-\ref{subsec_selective}, as it does not relate specifically to the \emph{estimated} latent variable vector. As jackstraw can only approximate the distribution of $\hat{\beta}\left(\hat{L}(X),{X}_j \right)$  under the null and not under any alternative, the jackstraw tests can not easily be inverted to construct confidence intervals for a parameter. 

Carrying out jackstraw as described above is computationally infeasible. It requires computing $\hat{L}(\cdot)$ for $B \times p$ different matrices.To get around this computational barrier, the jackstraw paper \cite{chung2015statistical} suggests a more efficient procedure in which $s$ genes are permuted in each of the $B$ iterations, and test statistics are computed for all $s$ permuted genes with respect to $\hat{L}(X^{permute,b})$. The $B \times s$ total test statistics are then compiled to form a single empirical null distribution, which is used to compute p-values for all $j$ genes. This strategy makes the strong assumption that the association between $X_j$ and $\hat{L}(X)$ that is attributable to double dipping is the same for $j=1,\ldots,p$. In Figure~\ref{fig_globalnull}, we see that this results in anti-conservative p-values for some genes and overly conservative p-values for others. Thus, while the set of all $p$ p-values appears to follow a $\text{Unif}(0,1)$ distribution, the marginals are incorrect, as discussed in 
\cite{leek2011joint} in a related setting. 

\subsection{PseudotimeDE}

\cite{song2021pseudotimede} recently proposed PseudotimeDE to test a gene's association with an estimated trajectory. Here we present a slight modification of their proposal tailored to our setting, and we describe the exact implementation details in Appendix~\ref{appendix_fig1help}. 

For $b=1,\ldots,B$, PseudotimeDE subsamples the cells in $X$ to obtain $X^b$, computes $\hat{L}(X^{b})$, and then permutes this vector to create $\hat{L}(X^{b})^{permute}$. It then computes $\hat{\beta}\left(\hat{L}(X^{b})^{permute}, X^b_j \right)$ for each of the $B$ subsamples. The empirical p-value for the $j$th gene is given by
\begin{equation}
\label{eq_pde}	
\frac{1}{B} \sum_{i=1}^B \bold{1}\left\{ 
\left| \hat{\beta}\left(\hat{L}(X^{b})^{permute}, X^b_j \right) \right| \geq \left| \hat{\beta}\left(\hat{L}(X), X_j \right) \right|\right\}.
\end{equation}
Permuting the pseudotime vectors destroys not only the relationship between $X_j$ and $\hat{L}(X_j)$ that may come from true signal, but also the relationship that comes from double dipping. The right-hand side of the inequality in \eqref{eq_pde} is a double-dipped coefficient while the left-hand side is not. While it is not entirely clear exactly what null hypothesis pseudotimeDE is designed to test, in the motivating example from Section~\ref{subsec_motivatingexample} where the entries of $\bold{X}_j$ are i.i.d. (and thus not differentially expressed across any latent variable), the p-values from \eqref{eq_pde} are stochastically smaller than a $\text{Unif}(0,1)$ distribution and do not control the Type 1 error (Figure \ref{fig_globalnull}).
 
 



